JITLine: A Simpler, Better, Faster, Finer-grained Just-In-Time Defect Prediction

A Just-In-Time (JIT) defect prediction model is a classifier to predict if a commit is defect-introducing. Recently, CC2Vec -- a deep learning approach for Just-In-Time defect prediction -- has been proposed. However, CC2Vec requires the whole dataset (i.e., training + testing) for model training, assuming that all unlabelled testing datasets would be available beforehand, which does not follow the key principles of just-in-time defect predictions. Our replication study shows that, after excluding the testing dataset for model training, the F-measure of CC2Vec is decreased by 38.5% for OpenStack and 45.7% for Qt, highlighting the negative impact of excluding the testing dataset for Just-In-Time defect prediction. In addition, CC2Vec cannot perform fine-grained predictions at the line level (i.e., which lines are most risky for a given commit). In this paper, we propose JITLine -- a Just-In-Time defect prediction approach for predicting defect-introducing commits and identifying lines that are associated with that defect-introducing commit (i.e., defective lines). Through a case study of 37,524 commits from OpenStack and Qt, we find that our JITLine approach is at least 26%-38% more accurate (F-measure), 17%-51% more cost-effective (PCI@20%LOC), 70-100 times faster than the state-of-the-art approaches (i.e., CC2Vec and DeepJIT) and the fine-grained predictions at the line level by our approach are 133%-150% more accurate (Top-10 Accuracy) than the baseline NLP approach. Therefore, our JITLine approach may help practitioners to better prioritize defect-introducing commits and better identify defective lines.

==> Makefile <==
FILE_NAME := paper

TEMP_FILES := \
	$(FILE_NAME).aux \
	$(FILE_NAME).bbl \
	$(FILE_NAME).log \
	$(FILE_NAME).blg \
	$(FILE_NAME).brf \
	$(FILE_NAME).out

SECTION_FILES = \
	paper.tex \
	sections/header.tex \
	sections/introduction.tex \
	sections/background.tex \
	sections/studydesign.tex \
	sections/results.tex \
	sections/threats.tex \
	sections/RQ1.tex \
	sections/RQ2.tex 

BIBTEX_FILES = \
	myref.bib \
	additionalref.bib 

GEN_FIGURES = \
	$(NULL)

# STATIC_FIGURES = \
# 	figure/overview.pdf 

DEBUG=no
ifneq '$(DEBUG)' 'yes'
LATEX_FLAGS="-interaction=batchmode"
endif

.DELETE_ON_ERROR:

################################################################################
# Main paper building
################################################################################
# $(STATIC_FIGURES)
$(FILE_NAME).pdf: $(SECTION_FILES) $(GEN_FIGURES) $(BIBTEX_FILES) 
	pdflatex $(LATEX_FLAGS) $(FILE_NAME)
	bibtex $(FILE_NAME)
	pdflatex $(LATEX_FLAGS) $(FILE_NAME)
	pdflatex $(LATEX_FLAGS) $(FILE_NAME)
	rm -f $(TEMP_FILES)
	open $(FILE_NAME).pdf
	# rm $(FILE_NAME).pdf


################################################################################
# Camera-Ready
################################################################################
.PHONY: camera
camera: 
	pdftops $(FILE_NAME).pdf
	ps2pdf14 -dPDFSETTINGS=/prepress $(FILE_NAME).pdf $(FILE_NAME)-new.pdf
	# pdffont $(FILE_NAME).pdf
	mv $(FILE_NAME)-new.pdf $(FILE_NAME).pdf
	open $(FILE_NAME).pdf
	# rm $(FILE_NAME).pdf
	
################################################################################
# Figures
################################################################################

#$(GEN_FIGURES): %.pdf: scripts/rms/analysis_figures.r scripts/rms/util.r
#	Rscript $<

################################################################################
# Clean
################################################################################
.PHONY: clean
clean:
	rm -f $(TEMP_FILES) $(GEN_FIGURES) $(FILE_NAME).pdf


==> sections/RQ1_old.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection*{\textbf{(RQ1) \rqi}}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % Table generated by Excel2LaTeX from sheet 'final exp result based on RQ'

% % \begin{table*}
% %   \caption{Experiment result of original work and our rerun model}
% %     \begin{tabular}{l|c|c|c|c|c|c|}
% % \cline{2-7}
% %  & \multicolumn{2}{c|}{Original Papers} & \multicolumn{2}{c|}{Ours} & \multicolumn{2}{c|}{\% Diff} \\
% % \cline{2-7} 
% %  & OpenStack & Qt & OpenStack & Qt & OpenStack & Qt \\
% % \hline
% %     DeepJIT & 0.751 & 0.768 & 0.75  & 0.76  & 0.13 & 1.04 \\
% %     CC2vec & 0.809 & 0.822 & 0.8   & 0.84  & 1.11 & 2.19 \\
% %     CC2vec (train only) & -     & -     & 0.77  & 0.81  & -     & - \\
% %     \hline
% %     \end{tabular}
% %   \label{tab:RQ1}
% % \end{table*}

% % Table generated by Excel2LaTeX from sheet 'final exp result based on RQ'
% \begin{table}[htbp]
%   \centering
%   \caption{Add caption}
%     \begin{tabular}{|c|c|c|c|}
%     \cline{3-4}    
%     \multicolumn{1}{r}{} &       & openstack & qt \\
%     \hline
%     \multirow{2}[2]{*}{DeepJIT (train only)} & original & 0.751 & 0.768 \\
%           & ours  & 0.75 & 0.76 \\
%     \hline
%     \multirow{2}[2]{*}{DeepJIT+Cc2vec (original)} & original & 0.809 & 0.822 \\
%           & ours  & 0.8 & 0.84 \\
%     \hline
%     \multirow{2}[2]{*}{DeepJIT+Cc2vec (train only)} & original & 0.77 & 0.81 \\
%           & ours  & -     & - \\
%     \hline
%     \end{tabular}%
%   \label{tab:RQ1}%
% \end{table}%



% \smallsection{Approach}
% We rerun source code of CC2Vec and DeepJIT with the same setting and dataset that are used in their work.
% However, we found that in CC2Vec implementation, test data is used to construct CC2Vec model.
% As a result, we correct CC2Vec experiment by excluding the test data and rerun source code again to check whether the experiment result of CC2Vec changes.

% \smallsection{Result}
% We successfully replicate the experiment result of DeepJIT and CC2Vec.
% The experiment result comparison between AUC, obtained from the authors' papers and ours, are presented in \ref{tab:RQ1}.
% % From the table, the percentage difference of Openstack and Qt result, obtained from DeepJIT, is 0.13 \% and 1.04 \% respectively.
% From the table, the difference between original result and our result, obtained from DeepJIT, is 0.13 \% for Openstack and 1.04 \% for Qt.
% Similarly, CC2Vec achieves similar results, having 1.11 \% and 2.19 \% difference in Openstack and Qt respectively.

% When looking at the result of CC2Vec which is trained with train data only, the AUC slightly drops for both Openstack and Qt.
% % I have no idea here T-T


==> sections/relatedwork.tex <==


% \section{Related Work}\label{sec:background}

% In this section, we discuss  several  Machine Learning (ML) and Deep Learning (DL) approaches for Just-In-Time defect prediction.

% \subsection{Machine Learning-based JIT defect prediction}
% Kim~\ea~\cite{Kim2008} are the first researchers that proposed machine learning model for JIT defect prediction. 
% In this work, they use support vector machine (SVM) to classify defective commits and clean commits. 
% The model is trained with code change metrics, complexity metric, Bag-of-Word, path names, and file names as features. 
% Later, Shivaji et. al \cite{Shivaji2013} apply feature selection techinque to improve the performance of this SVM model.
% Jiang et. al develop personalized JIT defect prediction model by using various machine learning techniques.
% They claimed that their proposed approach outperform the traditional machine learning model.
% Fukushima et. al \cite{Fukushima2014} proposed an ensemble machine learning, trained with code change metrics, for cross-project JIT defect prediction.
% They found that their approach can improve performance of such a task.
% Rajbahadur et. al \cite{Rajbahadur2017} present regression-based model for defective code change classification.
% The model works by predicting defect counts of a commit, then classify whether the commit is defective based on a specified threshold.
% The authors of this work also employ permutation feature importance to understand if their approach and traditional classification techniques learn with the same set of features.
% They discover that their approach outperforms the traditional approaches.



    % \subsection{Deep learning-based JIT defect prediction}
    
    % \kla{please add more details about CC2VEC and DeepJIT}
    
    % Recently, Wang et. al \cite{Wang2018} proposed deep belief network (DBN) with traditional classification model for within-project and cross-project defective code change prediction.
    % Firstly, DBN is used to extract features from code change, then the result of DBN is fed to classifier model to make a prediction.
    % They proved that their approach can improve performance in term of F1 measure.
    % Hoang et. al \cite{Hoang2019} proposed DeepJIT, a deep learning model for JIT defect prediction.
    % In this work, the authors employ two convolutional neural networks (CNN), one for extracting features from commit message, and the other one for code change features extraction.
    % The resulting vectors from both networks are then concatenated to form a final feature vector.
    % This vector is then fed to fully-connected layer to produce a prediction whether a given code commit is defective.
    % In this work, the authors employ convolutional neural network (CNN) to extract features from commit message and code change of a commit.
    % The extracted features are combined and fed to neural network layer to predict defective commits.
    % The experiment result confirms that DeepJIT outperforms traditional machine learning approach, which trained on code change metrics.
    % Later, they develop CC2Vec \cite{CC2Vec}, a hierarchical attention network (HAN) model that transforms code change to a vector representation.
    % The added code change and removed code change of a commit are separately fed to HAN model.
    % The features are extracted from each changed file of the commit.
    % After that the extracted feature vectors are used to create new features at comparison layer, which is composed of different functions defined by the authors.
    % The result of this layer are then concatenated to form a vector representing code change of the commit.
    % This vector is then used as a feature for DeepJIT to predict defective commits.
    % From the experiment result, the authors claimed that CC2Vec can improve DeepJIT's performance.
    

    % \subsection{Effort-aware JIT defect prediction}
    % Kamei et. al \cite{Kamei2013} proposed effort-aware logistic regression model for effort-aware JIT defect prediction.
    % They use change metrics as features for model training.
    % The experiment result confirmed that their proposed approach can reduce effort that software developers have to spend on code inspection.
    % Yang et. al \cite{Yang2016} presented an unsupervised machine learning model to predict defective commits.
    % The features used in the experiment are similar to the ones used in \cite{Kamei2013}.
    % They found that the result obtained from unsupervised model is competitive to the result of state-of-the-art supervised model.
    % Chen et. al \cite{Chen2018} developed a multi-objective optimization based supervised method called MULTI.
    % They built logistic regression model to achieve two objectives: maximizing the number of defective commits and minimizing the effort to inspect code change.
    % According to their experiment result, the proposed approach obtain better performance when compared to state-of-the-art supervised and unsupervised machine learning model in different evaluation measures.
    % Li et. al \cite{Li2020} proposed semi-supervised model namely Effort-Aware Tri-Training (EATT).
    % The model employs tri-training method with three machine learning classifiers to exploit unlabelled data.
    % The experiment result demonstrates that EATT can outperform existing state-of-the-art supervised and unsupervised model.

% \subsection{Effort-aware defect prediction}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/studydesign.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Case Study Design}\label{sec:design}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we describe the design of our case study experiment that we perform in order to address our research questions.
Figure~\ref{fig:overview} provides an overview of the approach that we apply to each studied system.
The crux of our approach is that we calculate a ground truth performance such that the performance estimates derived from model validation techniques can be compared against it.
We describe each step in the approach below.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Studied Systems}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In selecting the studied systems, we identified two important criteria that needed to be satisfied:

\begin{itemize}
\item \textbf{Criterion 1 --- Sufficient EPV}:
  Since we would like to study cases where EPV is low-risk (i.e, $\ge 10$) and high-risk ($< 10$), the systems that we select for analysis should begin with a low-risk EPV.
  Our rationale is that we prefer under-sampling to over-sampling when producing our sample dataset.
  For example, if we were to select systems with an initial EPV of 5, we would need to over-sample the defective class in order to raise the EPV to 10.
  However, the defective class of a system with an initial EPV of 15 can be under-sampled in order to lower the EPV to 10.

\item \textbf{Criterion 2 --- Sane defect data}:
  Since it is unlikely that more software modules have defects than are free of defects, we choose to study systems that have a rate of defective modules below 50\%.

\end{itemize}

We began our study using the 101 publicly-available defect datasets described in Section~\ref{sec:background}. 
To satisfy criterion 1, we exclude the 78 datasets that we found to have an EPV value lower than 10 in Section~\ref{sec:background}.
To satisfy criterion 2, we exclude an additional 5 datasets because they have a defective ratio above 50\%.
% (i.e., lucene-2.4, poi-2.5, poi-3.0, xalan-2.7, xerces-1.4)

Table~\ref{tb:studiedsystems} provides an overview of the 18 systems that satisfy our criteria for analysis.
To combat potential bias in our conclusions, the studied systems include proprietary and open source systems, with varying size, domain, and defective ratio.



==> sections/threats.tex <==
% First, we found that in most
% of the buggy changes, the ratio of buggy lines among all the
% added lines is smaller than 0.25; half of them is near 0.125.
% This data highlights the necessary for JIT defect localization,
% since it is impractical to inspect all the changed lines for each
% change with limited inspection effort. Second, using our approach, possibly buggy lines can be highlighted in an early
% stage (i.e., at check-in time), developers can inspect them
% early when they are still fresh with the context. The benefit is
% that developers can locate the defect by only inspecting a list
% of highly defective lines suggested by our approach. Third,
% there are two ways for building a localization model, i.e.,
% a clean model and a buggy model. Clean model might be
% better for most of the projects, since buggy code tends to be
% surprising compared to clean code. Fourth, when applying
% our approach on a new project, we can train the localization
% model by learning from multiple other available projects.


%  First, JIT defect localization
% is a real problem which can be the second phase after JIT
% defect identification. Solely investigating JIT defect identification might be insufficient, since developers cannot
% identify where is the defect. We believe that JIT defect
% localization can promote the use of JIT defect identification
% in practice. Second, software naturalness is effective for JIT
% defect localization. Currently, we build a simple solution
% using N-gram. Further advanced methods are expected for
% improving the performance. Third, both prior clean code
% and prior buggy code are potentially useful for JIT defect
% location. Prior clean code can be used to detect the defect
% which is surprising to clean code, while prior buggy code
% can be used to detect the defect which is similar to prior
% buggy code.





% Construct Validity
% - some defective lines are identified as clean
%     - how to solve this??
%     - we find bug-fixing commit from the commits of the next 6 months ??

% It is possible that the defective lines of defect-introducing commits are identified as clean lines, or even bug-fixing commits of the defect-introducing commits are not found.
% To mitigate this issue, we 


% - parameters of ML models have impact on classification result
%     - how to solve this??
%     - some work \cite{} shows that parameters of ML models have impact, but other work \cite{} shows that parameters of RF is insensitive to overall performance 

% External Validity
%     - use only 2 datasets (Openstack and Qt) in our experiment, but in reality there are plenty of large-scale opensource and commercial software -> not generalized
%     - not use feature selection technique ?? -> result may be different 


% Internal Validity
%     - only use LIME tecnique to generate line score, while there are other techniques that we do not explore in this study. -> result may be different
    
% On the other hand, the computation time of the deep learning approaches can be accelerated by using a high-end GPU hardware.
% We found that the model training time of the deep learning approaches on the GPU device is X\% relatively faster than using the CPU hardware, with an additional estimated GPU hardware cost of \$1,000.
% When considering the cost-benefits (i.e., the performance improvement and the computational cost), the benefits of our approach still outweigh the cost.
% \todo{thinking how to end this one?}
% \todo{say something like despite using the GPU, the computational time still x\% more than our approach that use CPU}.

% Recently, Rodríguez-Pérez~\ea~\cite{rodriguez2018reproducibility} raised concerns that there are different variants of the SZZ algorithm. 
% In this paper, we identified defect-introducing commits using CommitGuru~\cite{Rosen:2015:FSE}, which uses the complete SZZ algorithm~\cite{sliwerski2005changes}. The SZZ algorithm is commonly used in prior work on JIT defect prediction~\cite{kamei2012large, kamei2016studying,yathish2019affectedrelease}. 
% The algorithm first identify defect-fixing commits by matching commits with bug reports labeled as fixed in the issue tracking system,
% and then employ the ``diff'' and ``blame'' functionality of VCS to determine the defect-introducing lines, and locate the defect-introducing commit that modifies the defect-introducing lines.
% This variant has two common limitations.
% First, it is possible that some commits may not be linked or incorrectly linked to the issue reports.
% Second, it is possible that the ``diff'' and ``blame'' functionality may involve cosmetic changes, comment changes, or new blank lines.
% Future research should consider addressing these limitations with an improved variation of the SZZ algorithm.


% - randomisation \cite{liem2020run,liu2020replicability} + set seed to ensure that the results are reproducible
